GOALS-JWST: Small neutral grains and enhanced 3.3 micron PAH emission in the Seyfert galaxy NGC 7469

We present James Webb Space Telescope (JWST) Near Infrared Spectrograph (NIRSpec) integral-field spectroscopy of the nearby luminous infrared galaxy, NGC 7469. We take advantage of the high spatial/spectral resolution and wavelength coverage of JWST /NIRSpec to study the 3.3 um neutral polycyclic aromatic hydrocarbon (PAH) grain emission on ~60 pc scales. We find a clear change in the average grain properties between the star-forming ring and the central AGN. Regions in the vicinity of the AGN, with [NeIII]/[NeII]>0.25, tend to have larger grain sizes and lower aliphatic-to-aromatic (3.4/3.3) ratios indicating that smaller grains are preferentially removed by photo-destruction in the vicinity of the AGN. We find an overall suppression of the total PAH emission relative to the ionized gas in the central 1 kpc region of the AGN in NGC 7469 compared to what has been observed with Spitzer on 3 kpc scales. However, the fractional 3.3 um to total PAH power is enhanced in the starburst ring, possibly due to a variety of physical effects on sub-kpc scales, including recurrent fluorescence of small grains or multiple photon absorption by large grains. Finally, the IFU data show that while the 3.3 um PAH-derived star formation rate (SFR) in the ring is 8% higher than that inferred from the [NeII] and [NeIII] emission lines, the integrated SFR derived from the 3.3 um feature would be underestimated by a factor of two due to the deficit of PAHs around the AGN, as might occur if a composite system like NGC 7469 were to be observed at high-redshift.

==> tab1_PAH_Ne.tex <==
\begin{deluxetable*}{@{\extracolsep{4pt}}lccccccc}%{cccccccc}
\tabletypesize{\footnotesize}
\tablewidth{0pt}
 \tablecaption{PAH Band and Emission Line Fluxes }\label{tab:flux}

 \tablehead{
 \colhead{Regions} & \colhead{R.A.} & \colhead{Dec.} & \colhead{PAH 6.2\um} & \colhead{PAH 7.7\um} & \colhead{PAH 11.3\um} & \colhead{[NeII] 12.81\um} & \colhead{[NeIII] 15.56\um} \\
 \cline{4-6} \cline{7-8}
 \colhead{} & \colhead{(ICRS)} & \colhead{(ICRS)} & \multicolumn{3}{c}{($\times$10$^{-16}$ W/m$^{2}$)} & \multicolumn{2}{c}{($\times$10$^{-17}$ W/m$^{2}$)}\\ [-0.4cm]
%  \colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} & \colhead{(6)} & \colhead{(7)}  & \colhead{(8)}\\
 }
 \startdata 
R1  &  23:03:15.5147 & +8:52:25.111 & 5.31 $\pm$ 0.19 & 20.61 $\pm$ 1.04 & 4.80 $\pm$ 0.25 & 12.07 $\pm$ 0.16 & 1.14 $\pm$ 0.03 \\
R2  &  23:03:15.5791 & +8:52:24.734 & 4.72 $\pm$ 0.10 & 15.29 $\pm$ 0.61 & 4.34 $\pm$ 0.16 & 17.16 $\pm$ 0.13 & 1.28 $\pm$ 0.02 \\
R3  &  23:03:15.6279 & +8:52:25.076 & 3.64 $\pm$ 0.11 & 12.78 $\pm$ 0.74 & 3.24 $\pm$ 0.16 &  7.41 $\pm$ 0.08 & 1.44 $\pm$ 0.02 \\
R4  &  23:03:15.7021 & +8:52:25.267 & 3.65 $\pm$ 0.18 & 11.58 $\pm$ 0.86 & 3.28 $\pm$ 0.30 &  8.06 $\pm$ 0.06 & 1.03 $\pm$ 0.02 \\
R5  &  23:03:15.6789 & +8:52:25.999 & 4.04 $\pm$ 0.09 & 16.12 $\pm$ 0.58 & 3.83 $\pm$ 0.09 &  8.17 $\pm$ 0.07 & 2.54 $\pm$ 0.03 \\
R6  &  23:03:15.7192 & +8:52:26.531 & 3.36 $\pm$ 0.12 & 13.24 $\pm$ 0.64 & 3.51 $\pm$ 0.20 &  6.62 $\pm$ 0.05 & 0.95 $\pm$ 0.02 \\
R7  &  23:03:15.6853 & +8:52:27.197 & 3.71 $\pm$ 0.07 & 12.63 $\pm$ 0.40 & 4.02 $\pm$ 0.08 & 11.24 $\pm$ 0.07 & 1.14 $\pm$ 0.02 \\
R8  &  23:03:15.6422 & +8:52:27.714 & 3.29 $\pm$ 0.10 & 10.72 $\pm$ 0.52 & 2.69 $\pm$ 0.12 &  5.95 $\pm$ 0.04 & 0.68 $\pm$ 0.01 \\
R9  &  23:03:15.5919 & +8:52:27.380 & 4.35 $\pm$ 0.08 & 15.98 $\pm$ 0.53 & 3.61 $\pm$ 0.10 &  8.67 $\pm$ 0.07 & 1.30 $\pm$ 0.02 \\
R10 &  23:03:15.5482 & +8:52:26.884 & 3.54 $\pm$ 0.10 & 13.75 $\pm$ 0.76 & 3.24 $\pm$ 0.15 &  8.27 $\pm$ 0.07 & 1.29 $\pm$ 0.02 \\
R11 &  23:03:15.5096 & +8:52:26.217 & 3.74 $\pm$ 0.10 & 13.68 $\pm$ 0.57 & 3.62 $\pm$ 0.18 &  8.92 $\pm$ 0.06 & 1.02 $\pm$ 0.01 \\
R1a &  23:03:15.5366 & +8:52:25.419 & 6.37 $\pm$ 0.27 & 26.14 $\pm$ 1.58 & 6.77 $\pm$ 0.38 & 13.43 $\pm$ 0.18 & 2.55 $\pm$ 0.05 \\
R2a &  23:03:15.5881 & +8:52:25.210 & 6.18 $\pm$ 0.16 & 23.24 $\pm$ 1.02 & 5.79 $\pm$ 0.21 & 15.72 $\pm$ 0.13 & 2.05 $\pm$ 0.03 \\
R7a &  23:03:15.6621 & +8:52:26.797 & 3.68 $\pm$ 0.08 & 14.57 $\pm$ 0.53 & 3.88 $\pm$ 0.07 & 10.06 $\pm$ 0.08 & 2.53 $\pm$ 0.03 \\
R10a &  23:03:15.5728 & +8:52:26.578 & 2.22 $\pm$ 0.07 & 8.87 $\pm$ 0.31 & 2.27 $\pm$ 0.02 & 6.38 $\pm$ 0.08 & 2.83 $\pm$ 0.06 \\
R2b &  23:03:15.6011 & +8:52:25.619 & 6.16 $\pm$ 0.40 & 25.75 $\pm$ 2.36 & 6.16 $\pm$ 0.18 & 13.19 $\pm$ 0.18 & 7.50 $\pm$ 0.12 \\
R7b &  23:03:15.6401 & +8:52:26.555 & 2.24 $\pm$ 0.17 &  9.60 $\pm$ 0.76 & 1.48 $\pm$ 0.05 &  5.10 $\pm$ 0.08 & 5.48 $\pm$ 0.08 \\
Nucleus & 23:03:15.6155 & +8:52:26.180 & 1.59 $\pm$ 0.26 & 5.24 $\pm$ 0.31 & 0.87 $\pm$ 0.14 & 7.63 $\pm$ 0.28 & 12.19 $\pm$ 0.27
 \enddata

 \vspace{-0.5cm}
 %\tablecomments{}
\end{deluxetable*}

==> tab2_H2.tex <==
\begin{deluxetable*}{lccccccccccccc}
\tabletypesize{\footnotesize}
\tablewidth{0pt}
 \tablecaption{\molH\ Line Fluxes}\label{tab:h2_flux}

 \tablehead{
 \colhead{Regions} & \colhead{S(1)} & \colhead{S(2)} & \colhead{S(3)} & \colhead{S(4)} & \colhead{S(5)} & \colhead{S(6)} & \colhead{S(7)} \\ [-0.2cm] 
 \colhead{} & \colhead{17.04\um} & \colhead{12.28\um} & \colhead{9.67\um} & \colhead{8.03\um} & \colhead{6.91\um} & \colhead{6.11\um} & \colhead{5.51\um} \\ 
 [-0.4cm] 
 }
%\vspace{-10pt}
 \startdata 
R1  & 4.70 $\pm$ 0.33 & 2.55 $\pm$ 0.08 & 3.95  $\pm$ 0.17 & 1.65 $\pm$ 0.13 & 3.08  $\pm$ 0.10 & 0.50 $\pm$ 0.07 & 1.34 $\pm$ 0.05 \\
R2  & 4.63 $\pm$ 0.15 & 2.38 $\pm$ 0.09 & 3.43  $\pm$ 0.10 & 1.35 $\pm$ 0.09 & 2.55  $\pm$ 0.08 & 0.36 $\pm$ 0.10 & 0.98 $\pm$ 0.07 \\
R3  & 1.83 $\pm$ 0.53 & 1.80 $\pm$ 0.07 & 2.48  $\pm$ 0.11 & 0.97 $\pm$ 0.07 & 1.71  $\pm$ 0.08 & 0.33 $\pm$ 0.05 & 0.59 $\pm$ 0.06 \\
R4  & 4.29 $\pm$ 0.22 & 2.17 $\pm$ 0.07 & 3.20  $\pm$ 0.09 & 1.04 $\pm$ 0.06 & 1.98  $\pm$ 0.07 & 0.40 $\pm$ 0.03 & 0.82 $\pm$ 0.06 \\
R5  & 4.31 $\pm$ 0.30 & 2.52 $\pm$ 0.12 & 3.95  $\pm$ 0.15 & 1.71 $\pm$ 0.09 & 3.00  $\pm$ 0.12 & 0.55 $\pm$ 0.10 & 1.27 $\pm$ 0.08 \\
R6  & 4.80 $\pm$ 0.12 & 2.41 $\pm$ 0.09 & 3.28  $\pm$ 0.09 & 1.26 $\pm$ 0.06 & 2.24  $\pm$ 0.12 & 0.36 $\pm$ 0.06 & 0.88 $\pm$ 0.15 \\
R7  & 4.08 $\pm$ 0.20 & 2.25 $\pm$ 0.06 & 3.64  $\pm$ 0.08 & 1.36 $\pm$ 0.06 & 2.46  $\pm$ 0.09 & 0.45 $\pm$ 0.05 & 1.24 $\pm$ 0.13 \\
R8  & 3.76 $\pm$ 0.07 & 1.91 $\pm$ 0.06 & 3.25  $\pm$ 0.10 & 1.19 $\pm$ 0.06 & 2.09  $\pm$ 0.07 & 0.37 $\pm$ 0.10 & 0.91 $\pm$ 0.06 \\
R9  & 1.79 $\pm$ 0.58 & 2.20 $\pm$ 0.06 & 3.36  $\pm$ 0.19 & 1.49 $\pm$ 0.07 & 2.48  $\pm$ 0.09 & 0.43 $\pm$ 0.05 & 1.12 $\pm$ 0.07 \\
R10 & 3.31 $\pm$ 0.29 & 1.78 $\pm$ 0.07 & 2.73  $\pm$ 0.12 & 1.09 $\pm$ 0.06 & 1.86  $\pm$ 0.07 & 0.28 $\pm$ 0.05 & 0.88 $\pm$ 0.08 \\
R11 & 3.31 $\pm$ 0.13 & 1.69 $\pm$ 0.07 & 2.48  $\pm$ 0.14 & 0.96 $\pm$ 0.06 & 1.62  $\pm$ 0.08 & 0.31 $\pm$ 0.06 & 0.61 $\pm$ 0.07 \\
R1a & 9.74 $\pm$ 0.36 & 4.82 $\pm$ 0.14 & 7.81  $\pm$ 0.19 & 3.28 $\pm$ 0.14 & 5.36  $\pm$ 0.13 & 1.05 $\pm$ 0.12 & 2.55 $\pm$ 0.14 \\
R2a & 6.19 $\pm$ 0.24 & 3.14 $\pm$ 0.12 & 5.16  $\pm$ 0.20 & 2.34 $\pm$ 0.10 & 3.75  $\pm$ 0.13 & 0.52 $\pm$ 0.13 & 1.75 $\pm$ 0.11 \\
R7a & 4.44 $\pm$ 0.19 & 2.88 $\pm$ 0.08 & 4.86  $\pm$ 0.13 & 2.07 $\pm$ 0.09 & 3.83  $\pm$ 0.09 & 0.63 $\pm$ 0.05 & 1.73 $\pm$ 0.11 \\
R10a & 3.56 $\pm$ 0.48 & 3.29 $\pm$ 0.20 & 6.94 $\pm$ 0.36 & 3.24 $\pm$ 0.22 & 6.00 $\pm$ 0.22 & 1.16 $\pm$ 0.12 & 2.97 $\pm$ 0.10 \\
R2b & 4.15 $\pm$ 0.76 & 4.76 $\pm$ 0.55 & 10.11 $\pm$ 0.53 & 6.36 $\pm$ 0.46 & 12.44 $\pm$ 0.37 & 2.53 $\pm$ 0.21 & 6.80 $\pm$ 0.51 \\
R7b & 3.38 $\pm$ 0.71 & 2.20 $\pm$ 0.30 & 3.83  $\pm$ 0.25 & 2.61 $\pm$ 0.33 & 5.66  $\pm$ 0.07 & 1.14 $\pm$ 0.06 & 3.07 $\pm$ 0.57 \\
Nucleus & 3.79 $\pm$ 1.45 & 2.77 $\pm$ 1.29 & 6.01 $\pm$ 0.59 & 4.70 $\pm$ 0.52 & 10.89  $\pm$ 0.21 & 2.24 $\pm$ 0.14 & 6.22 $\pm$ 1.92 \\
 \enddata
 \tablecomments{All \molH\ pure rotational line fluxes are in unit of 10$^{-18}$ W/m$^{2}$.}
\end{deluxetable*}
